Vision Language Models Are Not (Yet) Spelling Correctors

Spelling correction from visual input poses unique challenges for vision language models (VLMs), as it requires not only detecting but also correcting textual errors directly within images. We present ReViCo (Real Visual Correction), the first benchmark that systematically evaluates VLMs on real-world visual spelling correction across Chinese and English. ReViCo contains naturally occurring errors collected from real-world image data and supports fine-grained evaluation at both image and token levels. Through comprehensive experiments on representative cascaded (Qwen) and native (InternVL) open-source models, as well as closed-source systems (GPT-4o, Claude), we show that current VLMs fall significantly short of human performance, particularly in correction. To address these limitations, we explore two solution paradigms: a Joint OCR-Correction pipeline and a Background Information enhanced approach, both of which yield consistent performance gains. Our analysis highlights fundamental limitations of existing architectures and provides actionable insights for advancing multimodal spelling correction.

==> table/backgroud_correct_example.tex <==
\begin{table*}[t]
\centering
\caption{Case study of different prompting strategies on background-sensitive examples.}
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{Picture} & \textbf{Model} & \textbf{Direct} & \textbf{Joint OCR--Correction} & \textbf{Background Information} \\
\hline
\raisebox{-0.45\totalheight}{\includegraphics[width=0.18\linewidth]{figure/bg_example1.jpg}} 
& GPT-4o & [``no error''] & [``no error''] & [(``处'', ``醋'')] \\
\cline{2-5}
& QwenVL-32B & [``no error''] & [``no error''] & [``no error''] \\
\hline
\raisebox{-0.45\totalheight}{\includegraphics[width=0.18\linewidth]{figure/bg_example2.jpg}} 
& GPT-4o & [(``得'', ``到'')] & [``no error''] & [(``伤'', ``桑''), (``肾'', ``葚'')] \\
\cline{2-5}
& QwenVL-32B & [``no error''] & [``no error''] & [``no error''] \\
\hline
\end{tabular}
\end{table*}

